Aggregate Power Flexibility in Unbalanced Distribution Systems

With a large-scale integration of distributed energy resources (DERs), distribution systems are expected to be capable of providing capacity support for the transmission grid. To effectively harness the collective flexibility from massive DER devices, this paper studies distribution-level power aggregation strategies for transmission-distribution interaction. In particular, this paper proposes a method to model and quantify the aggregate power flexibility, i.e., the net power injection achievable at the substation, in unbalanced distribution systems over time. Incorporating the network constraints and multi-phase unbalanced modeling, the proposed method obtains an effective approximate feasible region of the net power injection. For any aggregate power trajectory within this region, it is proved that there exists a feasible disaggregation solution. In addition, a distributed model predictive control (MPC) framework is developed for the practical implementation of the transmission-distribution interaction. At last, we demonstrate the performances of the proposed method via numerical tests on a real-world distribution feeder with 126 multi-phase nodes.

==> distributed_algorithm_derivation.tex <==

\section{Distributed Solver for Power Aggregation}

To make the power aggregation scalable and protect the private information of the participated DER appliances, the distributed solver is developed for the proposed power aggregation optimization models based on the predictor corrector proximal multiplier (PCPM) algorithm \cite{pcpm}.  This section takes the optimal power aggregation model as example and introduces the concrete distributed solution scheme. 

For explicit expression, the OPA model is rewritten in the following separated form.

\begin{subequations}
	\textbf{OPA Model:}
	\begin{align}
	\text{Obj.}  & \   \min_{\mb{y}_0,\mb{y}_k} \ \  -\sum_{t=1}^{T}\left(P_{0,t}^\wedge-P_{0,t}^\vee\right)  \\
	\text{s.t.} \  
	&\mb{v}_t^\wedge=\sum_{k=1}^{K} \mb{A}_k\mb{x}_{k,t}^\wedge+\mb{a}_t,\ \ \mb{v}_t^\vee=\sum_{k=1}^{K} \mb{A}_k\mb{x}_{k,t}^\vee+\mb{a}_t \\
	&\mb{i}_{L,t}^\wedge=\sum_{k=1}^{K} \mb{B}_k\mb{x}_{k,t}^\wedge+\mb{b}_t ,\ \, \mb{i}_{L,t}^\vee=\sum_{k=1}^{K} \mb{B}_k\mb{x}_{k,t}^\vee+\mb{b}_t \\
	&P_{0,t}^\wedge=\sum_{k=1}^{K}\mathbf{c}_k^\top\mathbf{x}_{k,t}^\wedge+m_t,\  P_{0,t}^\vee=\sum_{k=1}^{K}\mathbf{c}_k^\top\mathbf{x}_{k,t}^\vee+m_t   \\ 
	& \mb{y}_0=\left\{ \mb{v}_t^\wedge,\mb{v}_t^\vee,\mb{i}_{L,t}^\wedge, \mb{i}_{L,t}^\vee,P_{0,t}^\wedge,P_{0,t}^\vee \right\}_{t\in\mc{T}}\in \mc{Y}_0 \\
	& \mb{y}_k=\left\{\mb{x}_{k,t}^\wedge,\mb{x}_{k,t}^\vee \right\}_{t\in\mc{T}} \in \mc{Y}_k \quad \forall k\in\mc{K}
	\end{align}
\end{subequations}


\begin{subequations}
	\textbf{Compact Form of OPA Model:}
	\begin{align}
	\text{Obj.}  & \   \min_{\mb{y}_0\in\mc{Y}_0,\mb{y}_k\in\mc{Y}_k} \mb{h}^\top\mb{y}_0   \\
	\text{s.t.} &\quad  \mb{y}_0 = \sum_{k=1}^{K}\mb{H}_k\mb{y}_k + \mb{z}
	\end{align}
\end{subequations}

The augmented Lagrangian function is 
\begin{align*}
	L\left(\mb{y}_0,\mb{y}_k,\bm{\mu}\right) &= \mb{h}^\top\mb{y}_0 + \bm{\mu}^\top\left(  \sum_{k=1}^{K}\mb{H}_k\mb{y}_k + \mb{z}-\mb{y}_0 \right)\\
	 &+ \frac{\rho}{2}|| \sum_{k=1}^{K}\mb{H}_k\mb{y}_k + \mb{z}-\mb{y}_0||^2\\
	 & + \frac{1}{2\rho}\left(||\mb{y}_0-\hat{\mb{y}}_0 ||^2 + \sum_{k=1}^{K}||\mb{y}_k-\hat{\mb{y}}_k ||^2 \right)
\end{align*}
Given ${\mb{y}}_0^l,\hat{\mb{y}}_k^l,\bm{\mu}^l$, the iteration method is 
$$ (\mb{y}_0^l-\mb{y}_0^{l+1})/\rho = \mb{h} - \left[ \bm{\mu}^l + \rho \left( \sum_{k=1}^K\mb{H}_k\mb{y}_k^{l+1} + \mb{z} -\mb{y}_0^{l+1} \right) \right]
$$

$$ (\mb{y}_k^l-\mb{y}_k^{l+1})/\rho = \mb{H}_k^\top \left[ \bm{\mu}^l + \rho \left( \sum_{k=1}^K\mb{H}_k\mb{y}_k^{l+1} + \mb{z} -\mb{y}_0^{l+1} \right) \right]
$$

Then use the approximation
$$ (\mb{y}_0^l-\mb{y}_0^{l+1})/\rho = \mb{h} - \left[ \bm{\mu}^l + \rho \left( \sum_{k=1}^K\mb{H}_k\mb{y}_k^{l} + \mb{z} -\mb{y}_0^{l} \right) \right]
$$

$$ (\mb{y}_k^l-\mb{y}_k^{l+1})/\rho = \mb{H}_k^\top \left[ \bm{\mu}^l + \rho \left( \sum_{k=1}^K\mb{H}_k\mb{y}_k^{l} + \mb{z} -\mb{y}_0^{l} \right) \right]
$$
Define auxiliary dual variable $$\bm{\nu}^{l+1}=\bm{\mu}^l + \rho \left( \sum_{k=1}^K\mb{H}_k\mb{y}_k^{l} + \mb{z} -\mb{y}_0^{l} \right)$$

Then the iteration form for the primal variables are
\begin{align*}
\begin{split}
\mb{y}_0^{l+1}=\arg \min_{\mb{y}_0\in\mc{Y}_0} 
\mb{h}^\top\mb{y}_0 - {\bm{\nu}^{l+1}}^\top\mb{y}_0
 + \frac{1}{2\rho}||\mb{y}_0-\mb{y}_0^{l} ||^2 
\end{split}
\end{align*}

\begin{align*}
\begin{split}
\mb{y}_k^{l+1}=\arg \min_{\mb{y}_k\in\mc{Y}_k} 
 {\bm{\nu}^{l+1}}^\top\mb{H}_k\mb{y}_k^{l} 
 + \frac{1}{2\rho}||\mb{y}_k-\mb{y}_k^{l} ||^2 
\end{split}
\end{align*}

After that, update the dual variables with
 $$\bm{\mu}^{l+1}=\bm{\mu}^l + \rho \left( \sum_{k=1}^K\mb{H}_k\mb{y}_k^{l+1} + \mb{z} -\mb{y}_0^{l+1} \right)$$
 
 
\textbf{System Aggregator:}

\textbf{DER Appliance $\mb{k}$:}

\begin{algorithm}[H]
	\caption{Distributed Scheme for OPA Model}
		while loop
\end{algorithm}


